A Survey of Internet Censorship and its Measurement: Methodology, Trends, and Challenges

Internet censorship limits the access of nodes residing within a specific network environment to the public Internet, and vice versa. During the last decade, techniques for conducting Internet censorship have been developed further. Consequently, methodology for measuring Internet censorship had been improved as well. In this paper, we firstly provide a survey of network-level Internet censorship techniques. Secondly, we survey censorship measurement methodology. We further cover the censorship of circumvention tools and its measurement, as well as available datasets. In cases where it is beneficial, we bridge the terminology and taxonomy of Internet censorship with related domains, namely traffic obfuscation and information hiding. We further extend the technical perspective with recent trends and challenges, including human aspects of Internet censorship.

==> figures/mots.tex <==
\begin{figure}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[
    scale=2,
    node distance = 2cm and 5cm,
    block/.style = {draw, rectangle, minimum width=2.5cm, minimum height=1cm, align=center},
    server/.style = {draw, rectangle, minimum width=2.5cm, minimum height=1cm, align=center, fill=green!20},
    censor/.style = {draw, diamond, aspect=1.5, minimum width=1.5cm, minimum height=1cm, align=center, fill=red!20, text width=1.5cm}, % Diamond shape
    arrow/.style = {-Stealth, thick},
    dashed_arrow/.style = {-Stealth, thick, dashed},
    packet/.style = {font=\footnotesize}
]

% Nodes
\node[block] (client) {Client};
\node[server, right=of client] (server) {Legitimate Server};
\node[censor, below=of client] (censor_node) {Censor};
\node[server, right=of censor_node] (malicious_server) {Malicious Server};

% Arrows: Client -> Server (Initial Request)
\draw[arrow] (client.5) -- (server.west|-client.5) node[midway, above, packet] {(1) HTTP GET};

% Arrows: Censor Interception and Redirection
\draw[arrow, red] (censor_node) -- node[left, packet, text=red,align=center] {(2) TCP Segment\\(Redirect)} (client);
\draw[dashed_arrow, gray] (server.west|-client.-5) -- node[midway, below, packet, text=gray] {Original Response (Discarded)} (client.-5);

% Arrows: Client -> Malicious Server
\draw[arrow, bend right=10] (client) to node[pos=0.5, below, packet, align=center,yshift=0cm,fill=white] {(3) HTTP GET\\(to Malicious\\Server)} (malicious_server);
\draw[arrow,color=red] (malicious_server) to node[pos=0.5, above, packet, align=center,xshift=0.5cm] {(4) Malware/\\Exploit} (client);

% Censor observation arrow (optional, but clarifies the censor's role)
\draw[-Stealth, dashed, bend right=30] (censor_node) to node[midway, above, sloped, font=\footnotesize] {Observes} (client);

\end{tikzpicture}
}
\caption{Man-on-the-Side (MotS) attack. The client (1) initiates an HTTP request to the legitimate server.  The censor (2) intercepts the traffic and injects a TCP segment containing a (3) redirect to a malicious server.  The client's original request may reach the server, and the server will respond. However, the Censor's (4) response arives earlier and is thus considered a duplicate by the client and discarded.  The client then connects to the malicious server, which delivers malware or an exploit.}
\label{fig:mots-attack}
\end{figure}
